Neural Dialogue State Tracking with Temporally Expressive Networks

Dialogue state tracking (DST) is an important part of a spoken dialogue system. Existing DST models either ignore temporal feature dependencies across dialogue turns or fail to explicitly model temporal state dependencies in a dialogue. In this work, we propose Temporally Expressive Networks (TEN) to jointly model the two types of temporal dependencies in DST. The TEN model utilizes the power of recurrent networks and probabilistic graphical models. Evaluating on standard datasets, TEN is demonstrated to be effective in improving the accuracy of turn-level-state prediction and the state aggregation.

==> problem_bak.tex <==
\section{Problem Statement}

\subsection{State Space in Dialogue Systems}
%In a spoken dialog system, the dialog manager maintains a {\em state} as the system interacts with the user. The state at each turn of the dialogue is meant to capture the entire history of the dialogue in a succinct representation so as for the system to decide how to respond next.
%% In the most general setting, the state may capture the system-interpreted intention and interest that the user has expressed so far; it may also store all responses of the system so far, which would, for example,  allow the system not to repeat a previous response uninteresting to the user.   
%In this work, we follow the standard formulation of state, for example, as in~\cite{Mrksic:15}, where the state is considered to maintain the system's ``belief'' of the user's interest or intention and more general connotations that the state may include are left out of our considerations. For instance, ${\tt FOOD}$ being included in $\mathcal {S}$ indicates that the system considers the user's interests in particular food type.  

In a dialogue system, the state is represented as a set of {\em slot-value} pairs. Let $\mathcal{S}$ denote the set of all slots, which contains elements ${\tt FOOD}$, ${\tt PRICERANGE}$ and ${\tt AREA}$. 
% Each slot in $\mathcal {S}$ is meant to indicate a possible aspect in which the user may be interested.
% , using a pre-defined set of {\em slots} and associated {\em values}. Formally, let $\mathcal{S}$ denote the set of all slots. 
% For example, the slot set $\mathcal {S}$ may be taken as  $\{{\tt FOOD}, {\tt PRICERANGE}, {\tt AREA}\}$. Each slot in $\mathcal {S}$ is meant to indicate a possible aspect in which the user may be interested.  
%the state is usually represented as a set of {\em slot-value pairs}, using a pre-defined set of {\em slots}
%and a predefined set of {\em values} associated with each slot. 
%Formally, let $\mathcal{S}$ denote the set of all slots. For example, in a dialogue system allowing a user to find restaurants, the slot set $\mathcal {S}$ may be taken as  $\mathcal{S}:=\{{\tt FOOD}, {\tt PRICERANGE}, {\tt AREA}\}$. Each slot token in $\mathcal {S}$ is meant to indicate a possible aspect in which the user may be interested. For instance, ${\tt FOOD}$ being included in $\mathcal {S}$ indicates that the system considers that the user might be interested in a particular food type.  
% Similarly,  ${\tt PRICERANGE}$ included as a slot token indicates that the system considers the user might express his interest in a particular price range.   
For each slot $s\in \mathcal{S}$, we use $\mathcal {V}(s)$ to denote the set of all values associated with slot $s$. For example, the value set $\mathcal {V}({\tt FOOD})$ may include value tokens ${\tt italian}$, ${\tt french}$, ${\tt chinese}$, etc. Under this setting, a state configuration $x$ is then a {\em set} of slot-value pairs.
% , namely in the form of $\{(s, v): s\in \mathcal {S}, v\in \mathcal {V}(s)\}$.
For example, a state configuration can be $\{({\tt FOOD}, {\tt italian}), ({\tt PRICERANGE}, {\tt moderate})\}$. The set of all state configurations will be denoted by $\mathcal{X}$ and referred to as the {\em state space}.

The state space is {\em conflict-free}. For example, a state configuration can not contain both $({\tt FOOD}, {\tt chinese})$ and $({\tt FOOD}, {\tt italian})$.
%A state configuration $x\in \mathcal {X}$ is said to be conflict-free if for any $(s, v) \in x$, there exists no $v'\in \mathcal {V}(s)$ such that $v'\neq v$ and $(s, v') \in x$. A state space $\mathcal {X}$ is said to be conflict-free if every $x\in \mathcal {X}$ is conflict-free. A quick inspection of the datasets we work with in this paper suggests that the state spaces thereof are indeed conflict-free.
% the value set $\mathcal {V}({\tt PRICERANGE})$ may include value tokens ${\tt cheap}$, ${\tt expensive}$, ${\tt moderate}$, etc. 
%Under this setting, a state configuration $x$ is then a {\em set} of slot-value pairs, namely in the form of $\{(s, v): s\in \mathcal {S}, v\in \mathcal {V}(s)\}$. 
%For example, a state configuration can be $\{({\tt FOOD}, {\tt italian}), ({\tt PRICERANGE}, {\tt moderate})\}$
%; when this configuration is maintained by the system, it means that so far the system considers that the user is interested in finding Italian food at a moderate price and that the user's other intentions and interest (e.g., to eat in which area) are {\em unknown}.  
%The set of all state configurations will be denoted by $\mathcal{X}$ and referred to as the {\em state space}. Usually, the state space is structured in such a way that no ``conflicting'' slot-value pairs may co-exist in the same state configuration. For example, a state configuration, as a set, can not contain both $({\tt FOOD}, {\tt chinese})$ and $({\tt FOOD}, {\tt italian})$. We now more formally state this condition. 
% \begin{center}
% 	\begin{shadowbox}
% 		{\parbox{6.5cm}
% 			{ {\bf Conflict-Free} \\
%				A state configuration $x\in \mathcal {X}$ is said to be {\em conflict-free} if for any $(s, v) \in x$, there exists no $v'\in \mathcal {V}(s)$ such that $v'\neq v$ and $(s, v') \in x$. A state space $\mathcal {X}$ is said to be
%				{\em conflict-free} if every $x\in \mathcal {X}$ is conflict-free.
% 			}
% 		}
% 	\end{shadowbox}
% \end{center}
%Although this condition appears quite restrictive, it only requires redefining $\mathcal {V}(s)$ for some or every $s\in \mathcal {S}$ to turn a state space $\mathcal {X}$ with conflicts
%to a conflict-free one.  In fact, a quick inspection of the datasets we work with in this paper suggests that the state spaces thereof are indeed conflict-free. Thus from here after, we will restrict exclusively to conflict-free state spaces.
The conflict-free condition of state space $\mathcal {X}$ provides a great convenience in the representation of state configurations. To that end, we introduce an additional value token, ${\tt unknown}$. And define 
 \begin{eqnarray*}
 \mathcal{V}^*(s) &:= &\mathcal {V}(s)\cup \{\tt unknown\}\\
 \mathcal{V}^* &:=&\bigcup_{s\in \mathcal {S}} \mathcal {V}^*(s) 
 \end{eqnarray*}
 Then each state configuration $x$ can be regarded as a function mapping from $\mathcal {S}$ to $\mathcal{V}^*$. For example,
% For example, if $x=\{({\tt FOOD}, {\tt italian}), ({\tt PRICERANGE}, {\tt moderate})\}$, then $x$ is treated as a function on $\mathcal {S}$, 
\begin{equation}
 \label{eq:exampleState}
 x(s)= \left\{
 \begin{array}{ll}
    {\tt italian},  &s={\tt FOOD}  \\
    {\tt moderate},  & s={\tt PRICERANGE} \\
     {\tt unknown}, & s={\tt AREA}
 \end{array}
 \right.
\end{equation}
From here on we will treat each state in $\mathcal {X}$ as such a function. 
% Note that in this case, as a function on $\mathcal{S}$,  any state configuration $x$ has its value $x(s)\in \mathcal{V}^*(s)$.  Thus in this view, the state space $\mathcal{X}$ can be regarded as the space of all functions $x:\mathcal {S}\rightarrow \mathcal{V}^*$ such that $x(s)\in {\mathcal V}^*(s)$ for all $s\in \mathcal{S}$. 
 %In addition, if the state configuration $x$ is such that $x(s)={\tt unknown}$ for every $s\in \mathcal {S}$, we will write $x=\emptyset$, consistent with the set-theoretic notation of $x$. 
 
 
 
 
 
 
%  For later use, we also define the set of all slot-value pairs by $\mathcal {P}$, that is,  
%  \[
%  \mathcal {P}:= \{(s, v): s\in \mathcal {S}, v\in \mathcal{V}^*(s)\}.
%  \]
 
 %Alternatively, the state configuration may be treated as a list value tokens, such as $x=({\tt italian}, {\tt moderate}, {\tt unknown})$,  if the slots in $\mathcal {S}$ are ordered.  The length of the list is the size $|\mathcal{S}|$ of $\mathcal {S}$.

%% below was Chen Junfan's original. Commented out. 

% For each $s\in \mathcal{S}$, $V(s)\subseteq \mathcal{V}$ denotes the set of all values for slot $s$. We let $V_{i}(s)$ be the $i^{\rm th}$ value of slot $s$, and $V_{0}(s)={\em none}$ is a special value that indicates no value for slot $s$ is expressed. The space of slot-value pairs is $\mathcal{S}\times\mathcal{V}$. A slot-value pair $(s, v)$ is said to be valid if $v \in V(s)$. Note that not all slot-value pairs $(s, v)\in\mathcal{S}\times\mathcal{V}$ is valid, we simply denote the set of all valid $(s, v)$ pairs as $(\mathcal{S}\times\mathcal{V})^{*}$. 

% Let $\mathcal{X}$ be the state space. Any state $x \in \mathcal{X}$ is a subset of $(\mathcal{S}\times\mathcal{V})^{*}$. A state said to be valid is defined as follows. 
% \begin{center}
% 	\begin{shadowbox}
% 		{\parbox{6.5cm}
% 			{
% 				A state $x\subseteq (\mathcal{S}\times\mathcal{V})^{*}$ is valid if for any $(s, v)\in x$, $(s, v')\notin x$ for all $v'\neq v$.
% 			}
% 		}
% 	\end{shadowbox}
% \end{center}

%We denote the set of all valid states as $\mathcal{X}^{*}$.

\subsection{The Dialogue Process and State Tracking}
The dialogue system usually converses with the user in multiple turns. At the $t^{\rm th}$ turn ($t\ge 0$), let $x_t$ denotes the state configuration of the system. The system first generates an {\em action} $a_t$ based on previous state $x_{t-1}$ and uttering a sentence to the user. The user then responds with a sentence, referred to as the {\em user utterance} and denoted by $u_t$. 
%Here an action is the system's internal representation of the content of the sentence to be uttered. 
%Usually, an action is represented as a set of keywords or key phrases. For example, an action can be $\{food, area\}$, which means that the system requests the food type the user is interested in and the area of the restaurant the user expects.  
%Specifically, the action $a_t$ can be regarded as a {\em set} of sentences. 
%Upon hearing the system's utterance, the user responds with some sentences in natural language, referred to as the {\em user utterance} and denoted by $u_t$. 
%These sentences, usually treated as a sequence of words, are referred to as the {\em user utterance} and denoted by $u_t$. 
Based on $(a_t, u_t)$, the system first predicts the turn-level state $y_t$, which is meant to capture the {\em true} intention of the current utterance $u_t$ and $y_t$ is also an element in the state space $\mathcal{X}$. According to $y_t$ and the previous state $x_{t-1}$, the system computes the aggregated state $x_{t}$ through a deterministic procedure. We next describe this procedure.
% the system then updates its state configuration from $x_{t-1}$ to $x_t$ through a deterministic procedure. We next describe this procedure.
%More precisely, the state updating is based on predicting the immediate state $y_t$, which is also 
%an element in the state space $\mathcal{X}$. However, here $y_t$ should not be interpreted as state, rather it is meant to capture the {\em true} intention or interest of the user expressed in the current utterance $u_t$. 
%The role that the immediate state $y_t$ plays in a dialogue is for the system to update its state from $x_{t-1}$ to $x_t$ according to 

For any given $s$, we define an binary operator $\triangleleft$ on $\mathcal {V}^*(s)$ as follows. For any $v, v' \in \mathcal{V}^*(s)$,
\begin{equation}
v \triangleleft v' :=
\left\{
\begin{array}{cc}
     v, & {\rm if} ~v'={\tt unknown} \\
     v', & {\rm otherwise}
\end{array}
\right.
\end{equation}
% We note that the expression $v\triangleleft v'$ defines a rule which ``updates'' the value of $v$ according to $v'$, where the updating only occurs when $v'$ is not ${\tt unknown}$, otherwise $v\triangleleft v'$ remains as $v$. 
% With the operator $\triangleleft$ defined on every $\mathcal{V}^*(s)$, we can extend the operator $\triangleleft$ to any two elements $x, y\in \mathcal{X}$, where $x\triangleleft y$ is also an element in $\mathcal{X}$ in which for every $s\in \mathcal{S}$
We then extend the operator $\triangleleft$ to any two elements $x, y\in \mathcal{X}$, where $x\triangleleft y$ is also an element in $\mathcal{X}$ 
\begin{equation}
(x\triangleleft y)(s):=x(s)\triangleleft y(s).
\end{equation}
Using this notation, the aggregation of states is precisely according to 
\begin{equation}
    \label{eq:stateUpdate}
    x_t=x_{t-1} \triangleleft y_t.
\end{equation}
For example, if $x_{t-1}$ takes the configuration $x$ in (\ref{eq:exampleState}) and if $y_t$ is
\begin{equation}
 %\label{eq:exampleTurnLabel}
 y_t(s)= \left\{
 \begin{array}{ll}
    {\tt chinese},  &s={\tt FOOD}  \\
    {\tt unknown},  & s={\tt PRICERANGE} \\
     {\tt unknown}, & s={\tt AREA}
 \end{array}
 \right.
\end{equation}
The aggregated state $x_t$ is
\begin{equation}
 %\label{eq:exampleNewState}
 x_{t}(s)= \left\{
 \begin{array}{ll}
    {\tt chinese},  &s={\tt FOOD}  \\
    {\tt moderate},  & s={\tt PRICERANGE} \\
     {\tt unknown}, & s={\tt AREA}
 \end{array}
 \right.
\end{equation}
% For later use, we introduce an indicator function, denoted by $g$, for the $\triangleleft$ operator. Specifically, 
% for any $x, y, x' \in \mathcal {X}$, 
% \begin{equation}
%     g(x, y, x'):= \left\{
%     \begin{array}{ll}
%     1, & {\rm if}~ x\triangleleft y= x'\\
%     0, &{\rm otherwise}
%     \end{array}
%     \right.
% \end{equation}
We note that the above deterministic rule is used in GLAD for state aggregation. 

Due to the stochastic nature of the dialogue process, it can be characterized by a random process $\{(X_t, Y_t, A_t, U_t):t=1, 2, \ldots)\}$. The probability measure defining the random process will be denoted by ${\mathbb P}$. In the rest of the paper, random variables will be denoted by capitalized letters and their values will be denoted by corresponding lower-cased letters. 

%\subsection{The Dialogue State Tracking Problem}
In the dialogue state tracking problem, the probability measure ${\mathbb P}$ which defines the dialogue process is unknown. We are however given a set $\mathcal{R}$ of realizations drawn from ${\mathbb P}$, where each $r\in \mathcal {R}$ is a dialogue, given in the form of $\{(x^{(r)}_t, y^{(r)}_t, a^{(r)}_t, u^{(r)}_t):t=1, 2, \ldots)\}$. Let  $x_{<t}$ denotes $(x_1, x_2, \ldots, x_t)$ and assume similar notations for $y_{<t}$, $a_{<t}$ etc. The objective of DST is to develop a predictor of $X_t$ from historical observations $A_{<t}, U_{<t}$. Using a machine learning approach, this boils down to learning from $\mathcal {R}$ an estimation of 
${\mathbb P}\left(x_t|a_{<t}, u_{<t}\right)$ for every $t$. 
%The more practical setting of the DST problem (noise-DST) can be somewhat more complicated, where in each realization in $\mathcal{R}$, $u_t$ is not directly given. 
In practice, the user utterance $u_t$ may not be given. Instead, a set of noisy versions of $u_t$ is given, each obtained from an ASR system. We denote the set of noisy sentences as $\widetilde{u}_t$ . The learning problem then becomes estimating ${\mathbb P}\left(x_t|a_{<t}, \widetilde{u}_{<t}\right)$ for every $t$.

% This work directly tackles the noise-DST problem. 



==> review.tex <==
\section{Reviews}
\subsection{Reviewer1}

1. Wrong statements and notations

2. It lacks an important baseline without state accumulation, which uses dialogue states as the target of Turn Label Prediction. It is different with TEN-X Model.

3. In Figure 3, why do you choose to put TEN-X-wrong and TEN-correct together in one column? It is weird.

4. Do you have any result of TEN model without a pre-trained TEN-X model? Since I just claimed that we can not extract unique $y_t$ from $x_t$.

5. If you are using already given $y_t$ of DSTC2, how do you process act-types like "deny", "confirm" in the label of semantic parser?



\subsection{Reviewer2}

1. The first limitation, "Insufficient account for feature temporal dependency" might not be established. NBT and GLAD still have access to information from history.

2. TEN-X that trained with turn labels itself has already outperformed the best competitors. However, TEN-X is essentially similar to baselines like GLAD, etc. It is hard to tell the role of the factor graph model. What if adding factor graph to the baseline methods like NBT, GLAD?

3. The experiments, I think, are not convincing enough that TEN is able to address all the limitations mentioned in the paper. It is better to provide some concrete examples that TEN works well by solving these limitations.

4. What in essence the difference between TEN-X and other baselines? Some models like NBT still has updating mechanisms (both heuristic and learned) to capture uncertainties to some extent.	

\subsection{Reviewer3}

1. Why you use the average word embedding in the same position in N-best ASR results instead of the average sentence embedding/representation? Do you use ASR confidence scores?

2. Each action contains m phrases (line 444). Could you give some examples of phrases?

3. About Figure 3, I found difficult to understand what exactly is being presented.

4. It's claimed that the proposed model can model the dialogue dynamics and can capture the temporal dependencies. Could you give some examples and analysis about this in the experiment?

